Semantic foundations of equality saturation

Equality saturation is an emerging technique for program and query optimization developed in the programming language community. It performs term rewriting over an E-graph, a data structure that compactly represents a program space. Despite its popularity, the theory of equality saturation lags behind the practice. In this paper, we define a fixpoint semantics of equality saturation based on tree automata and uncover deep connections between equality saturation and the chase. We characterize the class of chase sequences that correspond to equality saturation. We study the complexities of terminations of equality saturation in three cases: single-instance, all-term-instance, and all-E-graph-instance. Finally, we define a syntactic criterion based on acyclicity that implies equality saturation termination.

==> core.tex <==

% \subsection*{Homomorphisms and the core}

In the Chase, we care about the core because it has the following properties:
\begin{itemize}
  \item It is universal, i.e., homomorphic to every model.
  \item It is minimal.
  \item It is unique (up to isomorphism).
  \item It can be computed by the core chase.
\end{itemize}

While the definition of a core comes from graph theory, 
 how the core is defined for infinite graphs is not standard.
We want a definition that preserves the above properties.


\begin{definition}
  Two graphs $G_1$ and $G_2$ are homomorphically equivalent if there are 
  homomorphisms $G_1\rightarrow G_2$ and $G_2\rightarrow G_1$.
\end{definition}

\begin{definition}
  Given a graph $G$, a retract of $G$ is a subgraph $H \subseteq G$ such that
  there is a homomorphism $G\rightarrow H$, and this homomorphism is called 
  a retraction.
\end{definition}

\begin{definition}
  A graph $G$ is a core if every retract $H$ is isomorphic to $G$.
\end{definition}

The standard definition of a retract requires the retraction 
 to be idempoent, i.e., $f|_H$ (restricting the domain of $f$ to $H$) is the identity.
This requirement is not necessary for finite graphs, 
 in the sense that either version always compute the same core up to isomorphism.
Consider a graph $G$ and its core $H$, computed by 
 a non-idempoent retraction $f$.
Because $H$ is a core, $f|_H$ must be an isomorphism, 
 so it must be a permutation of the vertices of $H$.
Because permutations on a finite set form a group, 
 some composition $f|_H^k$ must be the identity function, 
 and thus $f\circ f|_H^{k-1}$ is an idempoent retraction from $G$ to $H$.


==> old-background-on-chase.tex <==
In this section, we briefly review necessary backgrounds on databases and the chase.
Next, we will show the fundamental connections between equality saturation and the chase.

\subsection{The Chase Procedure}\label{sec:chase}

\mysubparagraph{Databases and conjunctive queries}

A relational database \emph{schema} is a tuple of relation names
$\mathcal{S}=(R_1,\ldots, R_m)$ with associated arities $\arity(R_i)$.
A database instance is a tuple of relation instances
$I=(R_1^I,\ldots, R_m^I)$, where $R_i^I\subseteq \dom^{\arity(R_i)}$
for some domain $\dom$.  In this paper we allow an instance to be
infinite.  We often view a tuple $\vec{a}$ in $R_i^I$ as an atom
$R_i(\vec{a})$, and view the instance $I$ as a set of atoms.  The
domain $\dom$ is the disjoint union of set of \emph{constants} and a
set of \emph{marked nulls}.

A \emph{conjunctive query} $\lambda(\vec{x})$ is a formula with free
variables $\vec{x}$ of the form
$R_1(\vec{x_1})\land\ldots\land R_k(\vec{x_k})$, where each
$\vec{x}_i$ is a tuple of variables from $\vec{x}$.  The
\emph{canonical database} of a conjunctive query consists of all the
tuples $R_i(\vec{x_i})$, where the variables $\vec{x}$ are considered
marked nulls.

Let $I$, $J$ be two database instances. A \emph{homomorphism} from $I$
to $J$, in notation $h:I \rightarrow J$, is a a function
$h:\dom(I)\rightarrow\dom(J)$ that is the identity on the set of
constants, and maps each atom $R(\vec{a})\in I$ to an atom
$R(h(\vec{a}))\in J$. The notion of homomorphism immediately
extends to conjunctive queries and/or database instances.  The output
of a conjunctive query $\lambda(\vec{x})$ on a database $I$ is defined
as the set of homomorphisms from $\lambda(\vec{x})$ to $I$.  We say
that a database instance $I$ \emph{satisfies} a conjunctive query
$\exists \vec{x} \lambda(\vec{x})$, denoted by
$I\models \exists \vec{x}\lambda(\vec{x})$, if there exists a
homomorphism $\lambda(\vec{x}) \rightarrow I$.

\mysubparagraph{Dependencies}

TGDs and EGDs describe semantic constraints between relations.
A TGD is a first-order formula of the form \(\lambda(\vec{x},\vec{y})\rightarrow \exists \vec{z}. \rho(\vec{x},\vec{z})\)
where $\lambda(\vec{x}, \vec{z})$ and $\rho(\vec{x}, \vec{y})$ are conjunctive queries with free variables
in $\vec{x}\cup\vec{y}$ and $\vec{x}\cup\vec{z}$.
An EGD is a first-order formula of the form \(\lambda(\vec{x})\rightarrow x_i=x_j\)
where $\lambda(\vec{x})$ is a conjunctive query with free variables in $\vec{x}$ and $\{x_i, x_j\}\subseteq \vec{x}$.

% \mysubparagraph{Solutions to dependencies}

Fix a set of TGDs and EGDs $\Gamma$.  If $I$ is a database instance
and $d \in \Gamma$, then a \emph{trigger} for $d$ in $I$ is a
homomorphism from $\lambda(\vec{x}, \vec{y})$ (resp.\
$\lambda(\vec x)$) to $I$.  An \emph{active trigger} is a trigger $h$
such that, if $d$ is a TGD, then no extension $h$ to a homomorphism
$h' :\rho(\vec{x},\vec{z}) \rightarrow I$ exists, and, if $d$ is an
EGD, then $h(x_i)\neq h(x_j)$.  We say that $I$ is model for $\Gamma$,
and write $I\models \Gamma$, if it has no active triggers.

Given $\Gamma$ and $I$ we say that some database instance $J$ is a
{\em model} for $\Gamma, I$, if $J\models \Gamma$ and there exists a
homomorphism $I \rightarrow J$.  $J$ is called \emph{universal model}
if there is a homomorphism from $J$ to every model of $\Gamma$ and
$I$.  Universal models are unique up to homomorphisms.  

\mysubparagraph{The chase}

The chase is a fixpoint algorithm for computing universal models.  It
has been shown useful for a number of data management tasks, including
data exchange, query containment checking, and semantic query
optimization.  We consider two variants of the chase here: the
\emph{standard chase} and the \emph{oblivious Skolem chase} (or simply
\emph{Skolem chase}).

The standard chase computes answers by deriving a sequence of
\emph{chase steps} until all dependencies are satisfied.  A chase
step, denoted as $I\xrightarrow[]{d, h} J$, takes as inputs an
instance $I$, a homomorphism $h$, and a dependency $d$, in which $h$
is an active trigger of $d$ in $I$, and produces an output instance
$J$ by adding some tuples (for TGDs) or collapsing some elements (for
EGDs).  Specifically, if $d$ is a TGD, the chase step extends $I$ with
the tuple $h'(\rho(\vec{x},\vec{z}))$, where $h'$ is an extension of
$h$ that maps the variables $\vec{z}$ on which $h$ is undefined to
fresh marked nulls.  If $d$ is an EGD, if $h(x_i)$ (or $h(x_j)$) is a
marked null, a chase step replaces in $I$ every occurrence of $h(x_i)$
with $h(x_j)$ (or $h(x_j)$ with $h(x_i)$).  If neither $h(x_i)$ nor
$h(x_j)$ is a marked null and $h(x_i)\neq h(x_j)$, then the chase
fails.  

% For both TGDs and EGDs, $h$ is no longer an active trigger of
% $d$ after the chase step.  \rw{Not obvious to me that triggers won't
%   reactivate. Maybe add either a short proof or a citation? Or just
%   remove the claim if it's not important.}

A standard chase sequence starting at $I_0$ is a sequence of
successful chase steps
$I_0\xrightarrow{d_1,h_1}I_1 \xrightarrow{d_2,h_2}\cdots$ that is
\emph{fair}: for all $i\geq 0$, for each dependency $d$ and active
trigger $h$ of $d$ in $I_i$, some $j\geq i$ must exist such that $h$
is no longer an active trigger of $d$ in $I_j$.  The \emph{result} of
a (possibly infinite) chase sequence is
$\bigcup_{i\geq 0} \bigcap_{j\geq i} I_j$~\cite{bench-chase}.  
% \rw{How do you intersect instances? 
% After applying a EGD, we'll replace some marked null with another 
%  in certain tuples. Simply taking the intersection would drop these tuples.}
A chase sequence is
\emph{terminating} if it ends with $I_n$ and $I_n\models \Gamma$, in
which case $I_n$ is the result of the chase sequence.  The standard
chase is non-deterministic: depending on the order of firing, the
chase sequence can be different.  Different chase sequences can even
differ on whether they terminate.


The Skolem chase, discussed in~\cite{marnette2009generalized}, differs
from the standard chase in several ways.  It first \emph{skolemizes}
each TGD
$d: \lambda(\vec{x},\vec{y})\rightarrow \exists
\vec{z}. \rho(\vec{x},z_1,\ldots, z_k)$ to
\( \lambda(\vec{x},\vec{y})\rightarrow
\rho(\vec{x},f^d_{z_1}(\vec{x}), \ldots, f^d_{z_k}(\vec{x})), \) where
each $f^d_{z_j}$ is an uninterpreted function from $\dom^{|\vec{x}|}$
to $\dom$.  The result of the Skolem chase, denoted as $\sklchase(\Gamma, I)$, is the least fixpoint of
the immediate consequence operator (ICO) of the Skolemized TGDs.  To
handle equality constraints, the Skolem chase applies
\emph{singularization} \cite{marnette2009generalized} to dependencies,
which replaces equality symbols in a rule with an \textit{Eq}
relation, joins reused variables with \textit{Eq}, and axiomizes
\textit{Eq} with rules for transitivity, reflexivity, and
symmetricity.

Both the standard chase and the Skolem chase produce a universal model
% \footnote{Fagin et al.~\cite{FAGIN200589} proved
% the finite chase to be universal. Benedikt et al.~\cite{bench-chase} and Cal\`i et al.~\cite{DBLP:journals/corr/abs-1212-3357}
% suggested the infinite chase to be universal as well. We provide a proof of this claim in \cref{sec:proof-chase-universal}.}
of $\Gamma, I$~\cite{FAGIN200589,bench-chase,marnette2009generalized}.

==> universal.tex <==
\section{Proof of the chase (finite or infinite) is universal}
\label{sec:proof-chase-universal}

\begin{lem}
  Given dependencies $\Gamma$ and a database instance $I$,
    if there is a model $K$ for $\Gamma$ and $I$, 
    there is a homomoprhism from the result of the chase to $K$.
\end{lem}

\begin{proof}
  Let $K$ be a model for $\Gamma$ and $I$, 
  and $I_0 \rightarrow I_1 \rightarrow \cdots$
  be a chase sequence of $\Gamma$ on $I$.
  We first show by induction that each $I_i$ in the sequence has a homomoprhism to $K$.
  When $i=0$, $I_0 = I$, and by definition there is a homomoprhism $I \rightarrow K$.
  In the inductive case, we assume there is a homomoprhism $h_i: I_i \rightarrow K$.
  $I_{i+1}$ may be produced from $I_i$ by chasing either a TGD or an EGD.
  An EGD only merges nulls, so the homomorphism is preserved.
  For a TGD $R_1(\vec{x_1}) \wedge \cdots \wedge R_k(\vec{x_k}) \rightarrow \exists \vec{z} . R(\vec{x}, \vec{z})$,
  let $R_1(t_1), \ldots R_k(t_k)$  be the witness tuples for the chase step, 
  and let $R(t_x, t_z)$ be the tuple added. 
  By our inductive hypothesis, $\forall i \in [0,k] : h(R_i(t_i)) \in K$, 
  and since $K$ is a model, there must exist a tuple $R(t_x', t_z') \in K$, 
  where $t_x' = h(t_x)$, 
  and we can extend the homomoprhism by mapping $t_z$ to $t_z'$.
  We have shown each $I_i$ has a homomorphism to $K$, and since union and intersection preserve homomoprhism, 
  the chase result is homomorphic to $K$.
\end{proof}

